Hessian-free Optimization for Learning Deep Multidimensional Recurrent Neural Networks

Multidimensional recurrent neural networks (MDRNNs) have shown a remarkable performance in the area of speech and handwriting recognition. The performance of an MDRNN is improved by further increasing its depth, and the difficulty of learning the deeper network is overcome by using Hessian-free (HF) optimization. Given that connectionist temporal classification (CTC) is utilized as an objective of learning an MDRNN for sequence labeling, the non-convexity of CTC poses a problem when applying HF to the network. As a solution, a convex approximation of CTC is formulated and its relationship with the EM algorithm and the Fisher information matrix is discussed. An MDRNN up to a depth of 15 layers is successfully trained using HF, resulting in an improved performance for sequence labeling.

==> contents/old.tex <==

%\caption{Arabic Offline Handwriting Recognition Results. The label error rate is shown for each network and each optimization methods. $A^B$ means stack of $B$ layers having $A$ hidden LSTM cells in each layer. In SGD, the $\epsilon$ is the learning rate, and $\mu$ is the momentum.}
\section*{A\quad Derivation of the Proposed Approximation from Fisher Information Matrix}
The derivative of the negative log probability of Eq.~\eqref{eq:prob_label} is given by 
\begin{equation}
%\frac{\partial \mathcal{L}(\textbf{a})}{\partial a^t_k}=y^t_k-\frac{1}{p(\textbf{z}|\textbf{a})}\sum_{u\in B(z,k)}
-\frac{\partial \log p(\textbf{z}|\textbf{a})}{\partial a^t_k}=y^t_k-\frac{1}{p(\textbf{z}|\textbf{a})}\sum_{u\in B(z,k)}
\alpha(t,u)\beta(t,u).
\end{equation}
where $\alpha(t,u),\beta(t,u)$ denote forward, backward variable respectively, and $B$ is the set of positions where label $k$ occurs in $\textbf{z}$ as $B(\textbf{z},k)=\{u:\textbf{z}_u=k\}$. The detailed derivation is referred in \cite{gravesbook}. For compact notation, let $Y^t$ denote a column matrix containing $y^t_k$ as its $k$-th element, and let $V^t$ denote a column matrix containing $v^t_k=\frac{1}{p(\textbf{z}|\textbf{a})}\sum_{u\in B(\textbf{z},k)} \alpha(t,u)\beta(t,u)$ as its $k$-th element.

Fisher information matrix is given by
\begin{align}
F&=\mathbb{E}_\textbf{x}\left [ \mathbb{E}_{\textbf{z}\sim p(\textbf{z}|\textbf{x})} \left [   \left( \frac{\partial \log p(\textbf{z}|\textbf{x},\theta) }{\partial \theta}   \right) \left( \frac{\partial \log p(\textbf{z}|\textbf{x},\theta) }{\partial \theta}   \right)^\top \right ] \right]
\end{align}
Since CTC assumes output probabilities at each timestep to be independent of those at other timesteps \cite{gravesbook}, its Fisher information matrix is given as the sum of every timesteps, so it follows
\begin{align}
F&=\mathbb{E}_\textbf{x}\left[\sum_t J_{\mathcal{N}_t}^\top \mathbb{E}_{\textbf{z}\sim p(\textbf{z}|\textbf{a})} \left [   \left( \frac{\partial \log p(\textbf{z}|\textbf{a}) }{\partial a^t}   \right) \left( \frac{\partial \log p(\textbf{z}|\textbf{a}) }{\partial a^t}   \right)^\top \right ]  J_{\mathcal{N}_t}\right]\\
&=\mathbb{E}_\textbf{x}\left [\sum_t J_{\mathcal{N}_t}^\top \mathbb{E}_{\textbf{z}\sim p(\textbf{z}|\textbf{a})} \left [   \left( Y^t-V^t \right) \left( Y^t-V^t \right)^\top \right ]  J_{\mathcal{N}_t}\right]\\
\label{eq:fisher_caclulation}
&=\mathbb{E}_\textbf{x}\left[\sum_t J_{\mathcal{N}_t}^\top \left(   Y^t {Y^t}^\top - Y^t\mathbb{E}_\textbf{z} \left [   V^t \right ]^\top - \mathbb{E}_\textbf{z} \left [   V^t \right ] {Y^t}^\top + \mathbb{E}_\textbf{z} \left [   V^t{V^t}^\top \right ]\right) J_{\mathcal{N}_t}\right  ]
\end{align}
where $Y^t$ and $V^t$ are defined above.

$\mathbb{E}_\textbf{z}[v^t_k]$ is calculated by
%\begin{equation}
%\mathbb{E}_\textbf{z}[v^t_k]=\mathbb{E}_{\textbf{z}\sim %p(\textbf{z}|\textbf{a})}\left[\frac{1}{p(\textbf{z}|\textbf{a})}\sum_{u\in B(\textbf{z},k)} %\alpha(t,u)\beta(t,u)\right]=\sum_{\textbf{z}} \sum_{u\in B(\textbf{z},k)} \alpha(t,u)\beta(t,u)=y_k^t.
%\end{equation}
\begin{align}
\mathbb{E}_\textbf{z}[v^t_k]&=\mathbb{E}_{\textbf{z}\sim p(\textbf{z}|\textbf{a})}\left[\frac{1}{p(\textbf{z}|\textbf{a})}\sum_{u\in B(\textbf{z},k)} \alpha(t,u)\beta(t,u)\right]\\
&=\sum_{\textbf{z}} \sum_{u\in B(\textbf{z},k)} \alpha(t,u)\beta(t,u)\\
&=y_k^t.
\end{align}


$\mathbb{E}_\textbf{z}[v^t_i v^t_j]$ is given by
\begin{align}\label{eq:vv}
\mathbb{E}_\textbf{z}[v^t_i v^t_j]&=\mathbb{E}_{\textbf{z}\sim p(\textbf{z}|\textbf{a})}\left[\frac{1}{p(\textbf{z}|\textbf{a})^2}\sum_{u\in B(\textbf{z},i)} \alpha(t,u)\beta(t,u)\sum_{u\in B(\textbf{z},j)} \alpha(t,u)\beta(t,u)\right]
\end{align}
Unfortunately Eq.~\eqref{eq:vv} is not calculated analytically in general, thus we consider the same condition in section \ref{subsec:condition}. By the assumption of one dominant path in a label, $\mathbb{E}_\textbf{z}[v^t_i v^t_j]=0$ for $i\neq j$. If the dominant path visits $i$ at time $t$, $\sum_{u\in B(\textbf{z},i)} \alpha(t,u)\beta(t,u) = p(\textbf{z}|\textbf{a})$, otherwise $\sum_{u\in B(\textbf{z},i)} \alpha(t,u)\beta(t,u) = 0$. Under this condition, Eq.~\eqref{eq:vv} turns into
\begin{equation}
\mathbb{E}_\textbf{z}[v^t_i v^t_j]=\delta_{ij}\sum_{\textbf{z}} \sum_{u\in B(\textbf{z},i)} \alpha(t,u)\beta(t,u)=\delta_{ij}y_i^t
\end{equation}
where $\delta_{ij}$ is Kronecker delta. By substituting $\mathbb{E}_\textbf{z}[V^t]=Y^t$ and $\mathbb{E}_\textbf{z}[V^t{V^t}^\top]=\text{diag}(Y^t) $ to Eq.~\eqref{eq:fisher_caclulation}, it gives
\begin{equation}
F= \mathbb{E}_\textbf{x}\left[\sum_t J_{\mathcal{N}_t}^\top  (  \text{diag}(Y^t) - Y^t{Y^t}^\top ) J_{\mathcal{N}_t}\right]
\end{equation}
which is the same form of Eq.~\eqref{eq:final_ctc_hessian} and Eq.~\eqref{eq:ggn_block}.





%Since $\mathbb{E}_\textbf{z}[v^t_i v^t_j]$ is not calculated analytically in general, we assume $y^t_k \in \{0,1\}$ for all $t$, $k$. In this case, $p(\textbf{z}'|\textbf{a})=1$ for only one label $\textbf{z}'$ corresponding the result from best path decoding given $\textbf{y}$, $p(\textbf{z}|\textbf{a})=0$ for the other labels. Then $\mathbb{E}_\textbf{z}[v_i v_j] = \delta_{ij}y_i$. By substituting $\mathbb{E}_\textbf{z}[V^t]=Y^t$, $\mathbb{E}_\textbf{z}[V^t{V^t}^\top]=\text{diag}(Y^t) $ to Eq.~\eqref{eq:fisher_caclulation}, it gives
%\begin{equation}
%F= \mathbb{E}_\textbf{x}\left[\sum_t J_{\mathcal{N}_t}^\top  (  \text{diag}(Y^t) - Y^t{Y^t}^\top ) J_{\mathcal{N}_t}\right]
%\end{equation}
%which is the same form of Eq.~\eqref{eq:final_ctc_hessian}.




%Table \ref{table:timit} shows the phoneme error rate (PER) on the core set for phoneme recognition. The improved performance according to depth can be observed for both optimization methods. The best PER for HF is 18.54\% at 15 layers , and the one for SGD is 18.46 \% at 10 layers, which are comparable performance to the one reported in \cite{graves13}. Considering the previous experiments \cite{graves13} in which the reported results are PER 18.6\% from the network with 3 layers having 3.8 million weights and PER 18.4\% from the network with 5 layers having 6.8 million weights, the benefit from deeper network is obvious in terms of the number of weight parameters, although this is not meant to be the definitive performance comparison due to different preprocessing.



%Considering PER 18.6\% for the network with 3 layers having 3.8M weights and 18.4\% for the network with 5 layers having 6.8M weights in the previous experiments \cite{graves13}, the benefit from deeper network is obvious in terms of the number of weight parameters, although this is not meant to be the definitive performance comparison due to different preprocessing.

\subsection{Non-Convexity of CTC}\label{subsec:ctc_non_convex}

Given an input vector $[x_1,\dots,x_k]$, the $k$-dimensional softmax function is defined by 
\begin{equation}\label{eq:element_softmax}
\begin{split}
y_i=\frac{\exp(x_i)}{\sum_{i'}\exp(x_{i'})} & \text{ where }i=1,\dots,k.
\end{split}
\end{equation}
Since $-\log \left(y_{i}\right)$ is convex \cite{mvp}, $y_{i}$ is log-concave. In general the sum of log-concave function is not log-concave \cite{convex}. As a result, the CTC objective is not convex in general because it contains the sum of softmax components in Eq.~\eqref{eq:prob_label}.
%Since Eq.~\eqref{eq:reform_ctc} is essentially the cross entropy loss function for a softmax output layer, the GGN matrix is given by
%\begin{equation}\label{eq:intermediate-gauss-newton}
%G=J^\top_{\mathcal{N}_c}  H_{\mathcal{L}_c} J_{\mathcal{N}_c}
%\end{equation}
%since $H_{\mathcal{L}_c}$ is positive semidefinite as discussed in the previous section.


%In this case, the linear part is selected upto output layer before applying the softmax activation function.

%Obviously the linear part for GGN is selected upto output layer before applying the softmax activation function. In this way, the GGN of Eq.~\eqref{eq:reform_ctc}, $G_{\mathcal{L}_c \circ \mathcal{N}_c}$, is equivalent to the Fisher information matrix for any networks using CTC objective, although it contains intractable calculation.
%Pascanu \cite{pascanu2013revisiting} has shown the identity of GGN matrix and Fisher information matrix  for the softmax with cross-entropy.

%In this section, we provide a rather straightforward derivation of HF optimization for MDRNN. There are two differences in the derivation compared with the one for normal feedforward or recurrent neural networks \cite{marten10, marten11}. One is obtaining a local quadratic approximation for MDRNN, and the other is to efficiently calculate the matrix-vector product used at each iteration of CG.

%At each iteration, HF performs the CG method while maintaining the constant local quadratic approximation during CG iterations to satisfy the conjugacy constraint of basis of the directions.


%It is common to use CG to minimize the quadratic objective above to utilize the complete curvature information and achieve computational efficiency. There needs to be an efficient way to compute $Gv$ for an arbitrary vector $v$ since CG requires the evaluation of $Gv$ several times during the iteration. For neural networks, there is an efficient way to compute $Gv$ proposed by \cite{mvp}, extending the work of \cite{roperator}. In Section~\ref{subsec:matrix_vector}, we provide details including the derivation of $\mathcal{R}$ operator to compute $Gv$ for MDRNN. 



%In addition, Graves \cite{graves13} has shown that the performance is further improved by stacking MDRNN as the network gets deeper up to depth of 5 with state-of-the-art performance in phoneme recognition.

 %The GGN approximation is discussed in Section \ref{subsec:convex_loss}.


%where $\delta_n = \theta-\theta_n$ is the direction we are looking for and $G$ is a local approximation to the curvature of $\mathcal{L}(\theta)$ at $\theta_n$, which is typically obtained by approximating the Hessian matrix by the generalized Gauss-Newton (GGN) discussed in Section \ref{subsec:convex_loss}.


%Since MDRNN is composed of differentiable components, applying the sum, product, and chain rules repeatedly starting from the input layer enables computing $\mathcal{R}_{v}(\mathcal{N}(\theta))$ throughout the whole network.
%One can rewrite $J_{\mathcal{N}}v$ as a differential operator $\mathcal{R}_{v}(\mathcal{N}(\theta))$ and utilize known properties of differential operators for efficient computation \cite{roperator}.

%Next, multiplication of $J_{\mathcal{N}}v$ by $H_{\mathcal{L}}$ can be done in a direct way by computing $H_{\mathcal{L}}$ in an efficient way.

==> contents/table.tex <==
\begin{table}[ht]
\caption{Experimental results on arabic offline handwriting recognition. The label error rates are presented with different depth of networks for each optimization method. $A^B$ means a stack of $B$ layers having $A$ hidden LSTM cells in each layer. For HF, `epochs' is the number of times of processing the whole data in the training set before the stopping criteria is fulfilled. For SGD, a fixed number of 1000 epochs has been processed. $\epsilon$ is the learning rate, and $\mu$ is the momentum.}
\label{table:arabic}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc|cc|cl}
\hline
networks & depth & weights & HF (\%) & epochs & SGD  (\%) & $\{\epsilon,\mu\}$ \\
\hline
2-10-50 & 3 &159,369& 6.10 & 76.41 & 9.57& \{$10^{-4}$,0.9\}\\
2-10-$21^3$ & 5 & 157,681 & 5.85 & 89.64 & 9.19 &    \{$10^{-5}$,0.99\}\\
2-10-$14^6$ & 8 & 154,209 & 4.98 & 139.02 & 9.70&    \{$10^{-4}$,0.95\}\\
2-10-$12^8$ & 10 & 154,153 & 4.95 & 85.50 & 9.34&   \{$10^{-4}$,0.95\}\\
2-10-$10^{11}$ & 13 & 150,169  & 4.50 & 97.44 & 10.63&  \{$10^{-4}$,0.9\}\\
2-10-$9^{13}$ & 15 & 145,417  & 5.70 & 83.70 & 12.00&    \{$10^{-5}$,0.99\}\\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

%\begin{table}[h]
\begin{table}[ht]
\caption{Experimental results on phoneme recognition using TIMIT corpus. PER is presented with different MDRNN architectures (Depth $\times$ Block $\times$ Cell/Block). $\sigma$ is the standard deviation of Gaussian weight noise. The other parameters are the same as in Table~\ref{table:arabic}.}
\label{table:timit}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cc|ccl|cl}
\hline
networks & weights & HF (\%) & epochs &$\{\sigma\}$ & SGD (\%) & $\{\epsilon,\mu,\sigma\}$\\
\hline
$3\times20\times10$ & 771,542 &  20.14 & 21.28 &\{0.03\} & 19.99 & \{$10^{-4}$,  0.9,  0.05 \}\\
$5\times15\times10$ & 795,752 &  19.18 & 29.72 &\{0.05\} & 19.60 & \{$10^{-5}$,  0.99,  0.04 \}\\
$8\times11\times10$ & 720,826 & 19.09 & 54.64 &\{0.05\} & 19.63 & \{$10^{-5}$,  0.99,  0.05 \}\\
$10\times10\times10$ & 755,822 & 18.79 & 59.72 &\{0.04\} & 18.46 & \{$10^{-5}$,  0.95,  0.04 \}\\
$13\times9\times10$ & 806,588 & 18.59 & 92.8 &\{0.05\} & 18.36 & \{$10^{-6}$,  0.99,  0.04 \}\\
$15\times8\times10$ & 741,230 & 18.48 & 47.2 &\{0.04\} & 18.77 & \{$10^{-5}$,  0.9,  0.04 \}\\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[ht]
\caption{Experimental results on different tasks. The label error rate for handwriting recognition and PER for phoneme recognition are presented with different depth of networks for each optimization method. In the column of `network', $A^B$ means stack of $B$ layers having $A$ hidden LSTM cells in each layer, and the architecture for phoneme recognition is represented by (Depth $\times$ Block $\times$ Cell/Block). $\epsilon$ and $\mu$ are the learning rate and the momentum for SGD optimization, respectively. $\sigma$ is the standard deviation of Gaussian weight noise. The best results are described with its parameters.}
\label{table:result}
\vskip 0.1in
\begin{center}
%\begin{small}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{l|c|cl||l|cl|cl}
\hline
\multicolumn{4}{l||}{Arabic Handwriting Recognition} & \multicolumn{4}{l}{TIMIT Phoneme Recognition} \\
\hline
network &  HF & SGD& $\{\epsilon,\mu\}$ &network& HF &$\{\sigma\}$ &  SGD & $\{\epsilon,\mu,\sigma\}$\\
\hline
2-10-50 & 6.10 & 9.57& \{$10^{-4}$,0.9\} &$3\times20\times10$ &  20.14& \{0.03\}& 19.99 & \{$10^{-4}$,  0.9, 0.05 \}\\
2-10-$21^3$ & 5.85 & 8.86&    \{$10^{-5}$,0.99\}&$5\times15\times10$ &  19.18& \{0.05\} & 19.60 & \{$10^{-5}$,  0.99,0.04 \}\\
2-10-$14^6$  & 4.98 & 9.70&    \{$10^{-4}$,0.95\}&$8\times11\times10$ & 19.09 & \{0.05\}& 19.43 & \{$10^{-5}$,  0.99, 0.05 \}\\
2-10-$12^8$  & 4.95 & 9.34&   \{$10^{-4}$,0.95\}&$10\times10\times10$ & 18.79 &\{0.04\} & 18.46 & \{$10^{-5}$,  0.95, 0.04\}\\
2-10-$10^{11}$  & 4.50 & 10.63&  \{$10^{-4}$,0.9\}&$13\times9\times10$ & 18.59&\{0.05\} & 18.36 & \{$10^{-6}$,  0.99, 0.04\}\\
2-10-$9^{13}$   & 5.70& 12.00&    \{$10^{-5}$,0.99\}&$15\times8\times10$ & 18.54& \{0.04\} & 18.77 & \{$10^{-5}$, 0.9, 0.04\}\\
\hline
\end{tabular}
\end{sc}
%\end{small}
\end{scriptsize}
\end{center}
\vskip -0.1in
\end{table}


